Skill or Luck? Return Decomposition via Advantage Functions

Learning from off-policy data is essential for sample-efficient reinforcement learning. In the present work, we build on the insight that the advantage function can be understood as the causal effect of an action on the return, and show that this allows us to decompose the return of a trajectory into parts caused by the agent's actions (skill) and parts outside of the agent's control (luck). Furthermore, this decomposition enables us to naturally extend Direct Advantage Estimation (DAE) to off-policy settings (Off-policy DAE). The resulting method can learn from off-policy trajectories without relying on importance sampling techniques or truncating off-policy actions. We draw connections between Off-policy DAE and previous methods to demonstrate how it can speed up learning and when the proposed off-policy corrections are important. Finally, we use the MinAtar environments to illustrate how ignoring off-policy corrections can lead to suboptimal policy optimization performance.

==> rebuttal.tex <==
\setcounter{figure}{0}
\begin{figure}
    \centering
    \includegraphics[width=.45\linewidth]{figs/minatar/norm_overall_deter.pdf}
    \includegraphics[width=.45\linewidth]{figs/minatar/norm_overall_stoch.pdf}
    \caption{Normalized training curves for the deterministic (left) and stochastic (right) environments. Results were aggregated over random seeds and all backup lengths. Lines and
shadings represent the means and 1 standard error of the means, respectively.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}
    \node[circle, draw, minimum size=.7cm] (s1) at (0.0,.7) {$1$}; 
    \node at (-1.7, .7) {$p(s_0{=}1)=0.9$}; 
    \node[circle, draw, minimum size=.7cm] (s2) at (0.0,-.7) {$2$}; 
    \node at (-1.7, -.7) {$p(s_0{=}2)=0.1$}; 
    \node (ru) at (2.5, .7) {$r_\mathtt{u}{=}1$}; 
    \node (rd) at (2.5, -.7) {$r_\mathtt{u}{=}0$}; 
    \node[circle, draw, minimum size=.7cm] (s3) at (1.5,0) {$3$}; 
    \node[circle, draw, minimum size=.7cm] (s4) at (3.0,0) {$4$};
    \node[circle, draw, minimum size=.7cm] (s5) at (5.0,.7) {$5$}; 
    \node[circle, draw, minimum size=.7cm] (s6) at (5.0,-.7) {$6$}; 
    \node[circle, draw, minimum size=.7cm] (s7) at (6.5, 0) {$7$}; 
    \draw[->] (s1) -- node[above=.2cm]{$r{=}0$}(s3);
    \draw[->] (s2) -- node[below=.2cm]{$r{=}0$}(s3);
    \draw[->] (s3) to [out=30, in=150] (s4);
    \draw[->] (s3) to [out=-30, in=-150] (s4);
    \draw[-] (s4) to (4.0, 0);
    \draw[->] (4.0, 0) -- (s5);
    \draw[->] (4, 0) -- (s6);
    \draw[->] (s5) -- node[above=.2cm]{$r{=}1$} (s7);
    \draw[->] (s6) -- node[below=.2cm]{$r{=}0$} (s7);
    % \node[inner sep=0pt] (result) at (5, -5)
    % {\includegraphics[width=.7\linewidth]{figs/classic/value_estimate_stoch.pdf}};
    \end{tikzpicture}
    \includegraphics[width=.75\linewidth]{figs/classic/value_estimate_stoch.pdf}
    \caption{Top: An MDP extended from Figure 1. 
    Instead of terminating at state 4, the agent stochastically transition to state 5 or 6 with equal probability.
    Both states 5 and 6 have a single action, with rewards 1 and 0, respectively.
    State 7 is the terminal state.
    Bottom: We compare the values (with uniform policy) estimated by DAE, Off-policy DAE (with learned transition probabilities), and Off-policy DAE (oracle, with known transition probabilities). Lines and shadings represent the average and one standard deviation of the estimated values over 1000 random seeds. The dashed line represents the true value $V(1)=V(2)=1$. }
    \label{fig:classic}
\end{figure}
